"I Apologize For Not Understanding Your Policy": Exploring the Specification and Evaluation of User-Managed Access Control Policies by AI Virtual Assistants

The rapid evolution of Artificial Intelligence (AI)-based Virtual Assistants (VAs) e.g., Google Gemini, ChatGPT, Microsoft Copilot, and High-Flyer Deepseek has turned them into convenient interfaces for managing emerging technologies such as Smart Homes, Smart Cars, Electronic Health Records, by means of explicit commands,e.g., prompts, which can be even launched via voice, thus providing a very convenient interface for end-users. However, the proper specification and evaluation of User-Managed Access Control Policies (U-MAPs), the rules issued and managed by end-users to govern access to sensitive data and device functionality - within these VAs presents significant challenges, since such a process is crucial for preventing security vulnerabilities and privacy leaks without impacting user experience. This study provides an initial exploratory investigation on whether current publicly-available VAs can manage U-MAPs effectively across differing scenarios. By conducting unstructured to structured tests, we evaluated the comprehension of such VAs, revealing a lack of understanding in varying U-MAP approaches. Our research not only identifies key limitations, but offers valuable insights into how VAs can be further improved to manage complex authorization rules and adapt to dynamic changes.

==> Tables/table-results-no-accuracy-EHR.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\caption{Results of Evaluating Different \policies on a Series of VAs (EHRs)}
\label{table-results-no-accuracy-ehrs}
\begin{tabular}{cccccccccccccccccc}
\hline
\rowcolor[HTML]{FFFFFF} 
\textbf{}                       & \textbf{}                     & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{ChatGPT}}                                                                      & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Google Gemini}}                                                               & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Microsoft Copilot}}                                                           & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Deepseek}}                                                                                             \\
\rowcolor[HTML]{FFFFFF} 
\textbf{}                       & \textbf{}                     & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Context}}    & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{No Context}} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Context}}   & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{No Context}} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Context}}   & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{No Context}} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Context}}                & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{No Context}}             \\
\rowcolor[HTML]{FFFFFF} 
\textbf{Question}               & \textbf{GT}                   & \textbf{R-1}                   & \textbf{R- 2}                  & \textbf{R-1}                   & \textbf{R-2}                   & \textbf{R-1}                  & \textbf{R-2}                   & \textbf{R-1}                   & \textbf{R-2}                   & \textbf{R-1}                   & \textbf{R-2}                  & \textbf{R-1}                   & \textbf{R-2}                   & \cellcolor[HTML]{FFFFFF}\textbf{R-1} & \cellcolor[HTML]{FFFFFF}\textbf{R-2} & \cellcolor[HTML]{FFFFFF}\textbf{R-1} & \cellcolor[HTML]{FFFFFF}\textbf{R-2} \\ \hline
\multicolumn{18}{c}{\textbf{INF Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\rowcolor[HTML]{FFFFFF} 
Q-EHR-1                         & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-EHR-2                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
Q-EHR-3                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
Q-EHR-4                         & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFCCC9}\FALSE & \TRUE                          & \TRUE                         & \cellcolor[HTML]{FFCCC9}\FALSE & \TRUE                          & \FALSE                         & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-EHR-5                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \cellcolor[HTML]{FFCCC9}\TRUE  & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{18}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Modified INF Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-1 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-2 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFCCC9}\FALSE & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-3 & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\cellcolor[HTML]{FFFFFF}Q-EHR-4 & \cellcolor[HTML]{FFFFFF}\TRUE & \cellcolor[HTML]{FFCCC9}\FALSE & \cellcolor[HTML]{FFCCC9}\FALSE & \cellcolor[HTML]{FFFFFF}\TRUE  & \cellcolor[HTML]{FFCCC9}\FALSE & \cellcolor[HTML]{FFFFFF}\TRUE & \cellcolor[HTML]{FFFFFF}\TRUE  & \cellcolor[HTML]{FFFFFF}\TRUE  & \cellcolor[HTML]{FFCCC9}\FALSE & \cellcolor[HTML]{FFFFFF}\TRUE  & \cellcolor[HTML]{FFFFFF}\TRUE & \cellcolor[HTML]{FFFFFF}\TRUE  & \cellcolor[HTML]{FFCCC9}\FALSE & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-5 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFCCC9}\FALSE & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{18}{c}{\cellcolor[HTML]{FFFFFF}\textbf{SEMI-UNROLL Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-1 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-2 & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-3 & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-4 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-5 & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{18}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Modified SEMI-UNROLL Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-1 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-2 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-3 & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-4 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-5 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{18}{c}{\cellcolor[HTML]{FFFFFF}\textbf{SEMI-RULE Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-1 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-2 & \FALSE                        & \cellcolor[HTML]{FFCCC9}\TRUE  & \FALSE                         & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFCCC9}\TRUE & \FALSE                         & \FALSE                         & \FALSE                         & \TRUE                          & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-3 & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFCCC9}\TRUE  & \FALSE                        & \cellcolor[HTML]{FFCCC9}\TRUE  & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-4 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-5 & \FALSE                        & \cellcolor[HTML]{FFCCC9}\TRUE  & \FALSE                         & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFCCC9}\TRUE & \cellcolor[HTML]{FFCCC9}\TRUE  & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFCCC9}\TRUE  & \FALSE                        & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{18}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Modified SEMI-RULE Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-1 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-2 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-3 & \FALSE                        & \FALSE                         & \FALSE                         & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFCCC9}\TRUE & \cellcolor[HTML]{FFCCC9}\TRUE  & \FALSE                         & \TRUE                          & \FALSE                         & \cellcolor[HTML]{FFCCC9}\TRUE & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-4 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}Q-EHR-5 & \TRUE                         & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & {\color[HTML]{000000} \TRUE}   & \TRUE                          & \TRUE                          & \TRUE                          & \TRUE                         & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\ \hline
\end{tabular}
\end{table*}

==> Tables/table-results-no-accuracy-SC.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\caption{Results of Evaluating Different \policies on a Series of VAs (Smart Cars).}
\label{table-results-no-accuracy-smart-cars}
\begin{tabular}{cccccccccccccccccc}
\hline
\rowcolor[HTML]{FFFFFF} 
\textbf{}                      & \textbf{}                     & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{ChatGPT}}                                                                   & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Google Gemini}}                                                             & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Microsoft Copilot}}                                                         & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Deepseek}}                                                                                             \\
\rowcolor[HTML]{FFFFFF} 
\textbf{}                      & \textbf{}                     & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Context}} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{No Context}} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Context}} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{No Context}} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Context}} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{No Context}} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Context}}                & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{No Context}}             \\
\rowcolor[HTML]{FFFFFF} 
\textbf{Question}              & \textbf{GT}                   & \textbf{R-1}         & \textbf{R- 2}                         & \textbf{R-1}           & \textbf{R-2}                           & \textbf{R-1}         & \textbf{R-2}                          & \textbf{R-1}          & \textbf{R-2}                            & \textbf{R-1}                           & \textbf{R-2}        & \textbf{R-1}                   & \textbf{R-2}                   & \cellcolor[HTML]{FFFFFF}\textbf{R-1} & \cellcolor[HTML]{FFFFFF}\textbf{R-2} & \cellcolor[HTML]{FFFFFF}\textbf{R-1} & \cellcolor[HTML]{FFFFFF}\textbf{R-2} \\ \hline
\multicolumn{18}{c}{\textbf{INF Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\rowcolor[HTML]{FFFFFF} 
Q-SC-1                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-2                         & \FALSE                        & \FALSE               & \FALSE                                & \FALSE                 & \FALSE                                 & \FALSE               & \cellcolor[HTML]{FFCCC9}\TRUE         & \FALSE                & \TRUE                                   & \FALSE                                 & \FALSE              & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-3                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-4                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFCCC9} 
\cellcolor[HTML]{FFFFFF}Q-SC-5 & \cellcolor[HTML]{FFFFFF}\TRUE & \FALSE               & \FALSE                                & \FALSE                 & \FALSE                                 & \FALSE               & \FALSE                                & \FALSE                & \FALSE                                  & \FALSE                                 & \FALSE              & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       \\ \hline
\multicolumn{18}{c}{\textbf{Modified INF Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
Q-SC-1                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-2                         & \TRUE                        & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFCCC9}\FALSE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-3                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-4                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-5                         & \FALSE                        & \FALSE               & \FALSE                                & \FALSE                 & \FALSE                                 & \FALSE               & \FALSE                                & \FALSE                & \FALSE                                  & \FALSE                                 & \FALSE              & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\ \hline
\multicolumn{18}{c}{\textbf{SEMI-UNROLL Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\rowcolor[HTML]{FFFFFF} 
Q-SC-1                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-2                         & \FALSE                        & \FALSE               & \FALSE                                & \FALSE                 & \FALSE                                 & \FALSE               & \FALSE                                & \FALSE                & \FALSE                                  & \FALSE                                 & \FALSE              & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-3                         & \TRUE                         & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                  & \TRUE                                  & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-4                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFCCC9} 
\cellcolor[HTML]{FFFFFF}Q-SC-5 & \cellcolor[HTML]{FFFFFF}\TRUE & \FALSE               & \FALSE                                & \FALSE                 & \cellcolor[HTML]{FFFFFF}\TRUE          & \FALSE               & \FALSE                                & \FALSE                & \cellcolor[HTML]{FFFFFF}\TRUE           & \FALSE                                 & \FALSE              & \FALSE                         & \cellcolor[HTML]{FFFFFF}\TRUE  & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFFFFF}\TRUE        \\ \hline
\multicolumn{18}{c}{\textbf{Modified SEMI-UNROLL Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\rowcolor[HTML]{FFFFFF} 
Q-SC-1                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-2                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \cellcolor[HTML]{FFCCC9}\FALSE & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-3                         & \TRUE                         & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                  & \TRUE                                  & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                 & \cellcolor[HTML]{FFCCC9}\FALSE          & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-4                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-5                         & \FALSE                        & \FALSE               & \FALSE                                & \FALSE                 & \FALSE                                 & \FALSE               & \FALSE                                & \FALSE                & \FALSE                                  & \FALSE                                 & \FALSE              & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\ \hline
\multicolumn{18}{c}{\textbf{SEMI-RULE Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\rowcolor[HTML]{FFFFFF} 
Q-SC-1                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                 & \cellcolor[HTML]{FFCCC9}\FALSE          & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-2                         & \FALSE                        & \FALSE               & \FALSE                                & \FALSE                 & \FALSE                                 & \FALSE               & \FALSE                                & \FALSE                & \cellcolor[HTML]{FFCCC9}\TRUE           & \FALSE                                 & \FALSE              & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFCCC9}\TRUE        & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-3                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                 & \cellcolor[HTML]{FFCCC9}\FALSE          & \cellcolor[HTML]{FFCCC9}\FALSE         & \TRUE               & \TRUE                          & \cellcolor[HTML]{FFCCC9}\FALSE & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-4                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFCCC9} 
\cellcolor[HTML]{FFFFFF}Q-SC-5 & \cellcolor[HTML]{FFFFFF}\TRUE & \FALSE               & \FALSE                                & \FALSE                 & \cellcolor[HTML]{FFFFFF}\TRUE          & \FALSE               & \FALSE                                & \FALSE                & \cellcolor[HTML]{FFFFFF}\TRUE           & \FALSE                                 & \FALSE              & \FALSE                         & \cellcolor[HTML]{FFFFFF}\TRUE  & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFFFFF}\TRUE        \\ \hline
\multicolumn{18}{c}{\textbf{Modified SEMI-RULE Format}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
Q-SC-1                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                 & \TRUE                                   & \cellcolor[HTML]{FFCCC9}\FALSE         & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-2                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \TRUE                                 & \TRUE                 & \TRUE                                   & \TRUE                                  & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFCCC9}\FALSE       & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-3                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                 & \cellcolor[HTML]{FFCCC9}\FALSE          & \cellcolor[HTML]{FFCCC9}\FALSE         & \TRUE               & \TRUE                          & \cellcolor[HTML]{FFCCC9}\FALSE & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFCCC9}\FALSE       \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-4                         & \TRUE                         & \TRUE                & \TRUE                                 & \TRUE                  & \TRUE                                  & \TRUE                & \cellcolor[HTML]{FFCCC9}\FALSE        & \TRUE                 & \TRUE                                   & \cellcolor[HTML]{FFCCC9}\FALSE         & \TRUE               & \TRUE                          & \TRUE                          & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        & \cellcolor[HTML]{FFFFFF}\TRUE        \\
\rowcolor[HTML]{FFFFFF} 
Q-SC-5                         & \FALSE                        & \FALSE               & \FALSE                                & \FALSE                 & \FALSE                                 & \FALSE               & {\color[HTML]{000000} \FALSE}         & \FALSE                & \FALSE                                  & \FALSE                                 & \FALSE              & \FALSE                         & \FALSE                         & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       & \cellcolor[HTML]{FFFFFF}\FALSE       \\ \hline
\end{tabular}
\end{table*}
